Interactive Topic Models with Optimal Transport

Topic models are widely used to analyze document collections. While they are valuable for discovering latent topics in a corpus when analysts are unfamiliar with the corpus, analysts also commonly start with an understanding of the content present in a corpus. This may be through categories obtained from an initial pass over the corpus or a desire to analyze the corpus through a predefined set of categories derived from a high level theoretical framework (e.g. political ideology). In these scenarios analysts desire a topic modeling approach which incorporates their understanding of the corpus while supporting various forms of interaction with the model. In this work, we present EdTM, as an approach for label name supervised topic modeling. EdTM models topic modeling as an assignment problem while leveraging LM/LLM based document-topic affinities and using optimal transport for making globally coherent topic-assignments. In experiments, we show the efficacy of our framework compared to few-shot LLM classifiers, and topic models based on clustering and LDA. Further, we show EdTM's ability to incorporate various forms of analyst feedback and while remaining robust to noisy analyst inputs.

==> figures/edtm-inference-partial.tex <==
\begin{algorithm}[t]
\small
    \caption{Complete topic assignment in \etmmethod}
    \begin{algorithmic}[1]
        \State \textbf{Input}: $D$, $L$, $f_{\text{dist}}$
%        \Comment{$f_{\text{dist}}$ bi/cross encoder distance function}
        \State $\mathbf{C} \gets f_{\text{dist}}(D,L)$ \Comment{Compute pairwise costs}
        \State $\mathbf{Q}^* \gets \text{zeros}(|D|, |L|)$ \Comment{Initialize plan with zeros}
        \For {epoch $e$ of $E$}
            \For {batch $b$ of $B$}
                \State $\mathbf{x}^b_D$, $\mathbf{x}_L \gets \text{uniform}(b), \text{uniform}(L)$
                \State $\mathbf{Q}^{*b} \gets \underset{\mathbf{Q}^b \in \mathcal{S}_c}{\texttt{argmin}}\langle\mathbf{C}^b,\mathbf{Q}^b\rangle - 1/\lambda H(\mathbf{Q}^b)$
                \State $\mathbf{Q}^*[b, :] \gets \mathbf{Q}^{*b}$ \Comment{Update plan for batch}
            \EndFor
        \EndFor
        \State $\mathbf{Q}^* \gets \mathbf{Q}^*/B\cdot E$ \Comment{Normalize plan}
        \State $\{l^*\}_{i=1}^{|D|} \gets \mathtt{argmax}_{l} \mathbf{Q}^*$
\end{algorithmic}
\label{alg-edtm-topicassign}
\end{algorithm}

==> figures/result-table-edtm-align.tex <==
\begin{table}
\centering 
\scalebox{1}{
\begin{tabular}{rrcccc}
\toprule
&  \multicolumn{2}{c}{Bookgenome} & \multicolumn{2}{c}{Bills} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
Method & {\footnotesize LDA} & {\footnotesize KMeans} & {\footnotesize LDA} & {\footnotesize KMeans}\\
\midrule
\etmmethodbe & & 2.17 & 1.1	& 1.24\\
\etmmethodce & & 1.83 & 1.19 & 1.22\\
& \multicolumn{2}{c}{Wiki} & \multicolumn{2}{c}{Twitter}\\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
\etmmethodbe & 1.03	& 0.94 & & 0.48\\
\etmmethodce & 1.27	& 1.11 & & 0.51\\
\bottomrule
\end{tabular}}
\caption{Mutual information between label supervised models and unsupervised models.}
\label{tab-edtm-align}
\end{table}

==> tex/07limits_impacts.tex <==
\section{Limitations}
\label{sec-limitations}
We dint do any human experiments.

\section{Ethical and Broader Impact}
\label{sec-eth-broad-impact}
Need to think about this.
